RadGenome-Chest CT: A Grounded Vision-Language Dataset for Chest CT Analysis

Developing generalist foundation model has recently attracted tremendous attention among researchers in the field of AI for Medicine (AI4Medicine). A pivotal insight in developing these models is their reliance on dataset scaling, which emphasizes the requirements on developing open-source medical image datasets that incorporate diverse supervision signals across various imaging modalities. In this paper, we introduce RadGenome-Chest CT, a comprehensive, large-scale, region-guided 3D chest CT interpretation dataset based on CT-RATE. Specifically, we leverage the latest powerful universal segmentation and large language models, to extend the original datasets (over 25,692 non-contrast 3D chest CT volume and reports from 20,000 patients) from the following aspects: (i) organ-level segmentation masks covering 197 categories, which provide intermediate reasoning visual clues for interpretation; (ii) 665 K multi-granularity grounded reports, where each sentence of the report is linked to the corresponding anatomical region of CT volume in the form of a segmentation mask; (iii) 1.3 M grounded VQA pairs, where questions and answers are all linked with reference segmentation masks, enabling models to associate visual evidence with textual explanations. All grounded reports and VQA pairs in the validation set have gone through manual verification to ensure dataset quality. We believe that RadGenome-Chest CT can significantly advance the development of multimodal medical foundation models, by training to generate texts based on given segmentation regions, which is unattainable with previous relevant datasets. We will release all segmentation masks, grounded reports, and VQA pairs to facilitate further research and development in this field.

==> content/03-datarecords.tex <==

\section*{Data Records}
\textbf{LOWER PRIORITY}
\xiaoman{each data record associated with this work, where this information is stored, and to provide an overview of the data files and their formats. Tables should be used to support the data records, and should clearly indicate the samples and subjects (study inputs), their provenance, and the experimental manipulations performed on each (please see 'Tables' below). They should also specify the data output resulting from each data-collection or analytical step, should these form part of the archived record.}


% \begin{figure}[tbh]
% \centering
% \includegraphics[width=\linewidth]{figure/dataset_abnormality_statistic.pdf}
% \caption{\xiaoman{update later}}
% \label{fig:dataset_overview}
% \end{figure}



==> content/04-technicalvalidation.tex <==

\section*{Technical Validation}
% \xiaoman{This section presents any experiments or analyses that are needed to support the technical quality of the dataset.}


% \subsection*{Benchmark Results}

==> content/06-ack.tex <==
\noindent LaTeX formats citations and references automatically using the bibliography records in your .bib file, which you can edit via the project menu. Use the cite command for an inline citation, e.g. \cite{Kaufman2020, Figueredo:2009dg, Babichev2002, behringer2014manipulating}. For data citations of datasets uploaded to e.g. \emph{figshare}, please use the \verb|howpublished| option in the bib entry to specify the platform and the link, as in the \verb|Hao:gidmaps:2014| example in the sample bibliography file. For journal articles, DOIs should be included for works in press that do not yet have volume or page numbers. For other journal articles, DOIs should be included uniformly for all articles or not at all. We recommend that you encode all DOIs in your bibtex database as full URLs, e.g. https://doi.org/10.1007/s12110-009-9068-2.

\section*{Acknowledgements} (not compulsory)

Acknowledgements should be brief, and should not include thanks to anonymous referees and editors, or effusive comments. Grant or contribution numbers may be acknowledged.

\section*{Author contributions statement}

Must include all authors, identified by initials, for example:
A.A. conceived the experiment(s), A.A. and B.A. conducted the experiment(s), C.A. and D.A. analysed the results. All authors reviewed the manuscript. 

\section*{Competing interests} (mandatory statement)

The corresponding author is responsible for providing a \href{https://www.nature.com/sdata/policies/editorial-and-publishing-policies#competing}{competing interests statement} on behalf of all authors of the paper. This statement must be included in the submitted article file.


==> content/07-figures_tables.tex <==
\section*{Figures \& Tables}

% Figures, tables, and their legends, should be included at the end of the document. Figures and tables can be referenced in \LaTeX{} using the ref command, e.g. Figure \ref{fig:stream} and Table \ref{tab:example}. 

% Authors are encouraged to provide one or more tables that provide basic information on the main ‘inputs’ to the study (e.g. samples, participants, or information sources) and the main data outputs of the study. Tables in the manuscript should generally not be used to present primary data (i.e. measurements). Tables containing primary data should be submitted to an appropriate data repository.

% Tables may be provided within the \LaTeX{} document or as separate files (tab-delimited text or Excel files). Legends, where needed, should be included here. Generally, a Data Descriptor should have fewer than ten Tables, but more may be allowed when needed. Tables may be of any size, but only Tables which fit onto a single printed page will be included in the PDF version of the article (up to a maximum of three). 

% Due to typesetting constraints, tables that do not fit onto a single A4 page cannot be included in the PDF version of the article and will be made available in the online version only. Any such tables must be labelled in the text as ‘Online-only’ tables and numbered separately from the main table list e.g. ‘Table 1, Table 2, Online-only Table 1’ etc.

% \begin{figure}[ht]
% \centering
% \includegraphics[width=\linewidth]{figure/dataset_overview.pdf}
% \caption{Legend (350 words max). Example legend text.}
% \label{fig:dataset_overview}
% \end{figure}


% \begin{figure}[ht]
% \centering
% \includegraphics[width=\linewidth]{figure/dataset_pipeline.pdf}
% \caption{Data construction pipeline of \OURDATA.}
% \label{fig:dataset_pipeline}
% \end{figure}

% \begin{table}[thb]
% \centering
% \begin{tabular}{llll}
% \toprule
% Level & Question type & Answer type & Example \\
% \midrule
% Patient & Disorders & Close/Open &  What diseases does this patient have? \\
% Region & Abnormality &  Open &  What abnormality is seen in the {region}? \\
% Region & Presence & Close &   Is there evidence of {abnormality} in this image? \\
% Region & Location & Close\&Open & Where in the image is the {abnormality}? \\
% Region & Size & Open & What is the size of the {abnormality} in this image? \\
% \bottomrule
% \end{tabular}
% \caption{\label{tab:datatype} Question and answer types in the proposed datasets }
% \end{table}

